Utility-Aware Load Shedding for Real-time Video Analytics at the Edge

Real-time video analytics typically require video frames to be processed by a query to identify objects or activities of interest while adhering to an end-to-end frame processing latency constraint. Such applications impose a continuous and heavy load on backend compute and network infrastructure because of the need to stream and process all video frames. Video data has inherent redundancy and does not always contain an object of interest for a given query. We leverage this property of video streams to propose a lightweight Load Shedder that can be deployed on edge servers or on inexpensive edge devices co-located with cameras and drop uninteresting video frames. The proposed Load Shedder uses pixel-level color-based features to calculate a utility score for each ingress video frame, which represents the frame's utility toward the query at hand. The Load Shedder uses a minimum utility threshold to select interesting frames to send for query processing. Dropping unnecessary frames enables the video analytics query in the backend to meet the end-to-end latency constraint with fewer compute and network resources. To guarantee a bounded end-to-end latency at runtime, we introduce a control loop that monitors the backend load for the given query and dynamically adjusts the utility threshold. Performance evaluations show that the proposed Load Shedder selects a large portion of frames containing each object of interest while meeting the end-to-end frame processing latency constraint. Furthermore, the Load Shedder does not impose a significant latency overhead when running on edge devices with modest compute resources.

==> contents/algo_old.tex <==

\subsection{Terminology}
%\begin{itemize}
%    \item A frame is represented by a \textbf{histogram} of HSV-values.
%    \item Each color-value is assigned a specific \textbf{bin}. The number of the bin is the color's \textbf{class}.
%    \item Each class for each color has a \textbf{color-utility}.
%    \item A frame's utility is the maximum of all color-utilities.
%    \item The utility-threshold for a \textbf{required shedding ratio} can be taken from the \textbf{utility-CDF}. 
%\end{itemize}
\todo{Add notations in a table}
\subsection{Overview}
Our load-shedding approach is utility-driven: 
To control load on the operator, the load shedder holds a \textit{utility threshold}.
Then a pre-trained model assigns a utility-value to each arriving frame.
If the frame's utility is below this threshold, the frame is dropped.

We show in the following how we compute a frame's utility, which includes how we train the utility model from the color distributions in a sample data-set.
We further explain how the shedder's utility threshold is calculated to achieve a required shedding rate. 

The steps of our solution are as follows: 
We first train a model that assigns utilities to frames. 
This model uses the color-distribution within the frame. 
It permits for a fast utility-lookup at runtime. This ensures that the shedding keeps low overhead. 
Then we compute the utility-distribution within the sample data-set.
From this distribution, we compute the mentioned utility threshold. 
Finally, at runtime, we use the model to look up a frame's utility and make the shedding decision.

\subsubsection{Utility}
In general, we compute the utility of frames in a sample data-set as shown in Equation  \ref{eq:utility_computation}.

\begin{equation}
\label{eq:utility_computation}
    u = \frac{\sum_{samples | L(sample) = 1}}{ \sum_{samples}}.
\end{equation}

For example assume 20 frames.
5 frames are labelled 1, 15 are labelled 0. The resulting utility is $5/20 = 0.25$.

However, we aim to give samples with a higher matching-probability for the given query a higher utility and those with a lower matching-probability a lower one respectively. 
The general idea is that if a query searches for objects of a certain color, we expect a minimum amount of pixels of this color in those frames that match the query.

Therefore, in the following, we use a frame's color distribution to determine a frame's utility more fine-grained and compute the utilities of all frames in the sample data-set.

Having the utilities of all frames in the sample data-set, we compute the overall utility distribution. 
From this distribution, we look up the utility threshold that the load shedder uses runtime to decide whether to shed a frame or to keep it. 

In the following, we first explain how we map video frames and their color distribution to color-wise utilities. Then we show how we thereof derive the frame's overall utility, and how we finally compute the overall utility distribution and the respective utility threshold. 

\subsubsection{Training Data}
To train the utility-models, we use a labeled stream of videos from multiple cameras as training data set. 
For each frame, a label and a HSV histogram are provided. 
The label tells whether there has been an object of interest in the frame, i.e., whether the frame was a match for the given query.
The HSV histogram holds the sum for each H (hue), S (saturation) and V (value for brightness) value in the frame.

Please note that we extract the HSV histogram from foreground information, only. This ensures that we only capture information about moving objects as those are the objects of interest for the queries.

\textit{Align with query definitions so that motivation for Hue-value fits.}

\subsection{Training of a Utility Model}
The utility model assigns a utility value to each frame based on the frame's color distribution. 
To this end, the frame's hue values are grouped by colors. 
From  there, each color is assigned a bin depending on the color's frequency in the frame. Finally, the bins are merged into classes per color and for each class, a utility value is computed.

\subsubsection{Mapping of Video-Frames to Utility Classes per Color}
\textit{Maybe add that to the application?! At least how the HSV values are used for object detection. Query will cover these same colors.}

In the system model provided, a developer can choose from twelve colors. 

\textit{pls verify that it's really 12!!!!}

The colors are defined by a range of HSV-values.
Only the H-ranges are non-overlapping and thus legible for classification.
For training, we therefore use each frame's H values which is an array of 256 entries and define a mapping $f: H \rightarrow C$ with $H = \mathbb{N}^{256}$ and $C = \mathbb{R}^{12}$. 
f sums up the hue-counts per color. 

The total number of pixels counted in each histogram can differ because the histogram reports foreground-pixels in the frame, only. The color count $C$ is thus relative, i.e., we divide the hue-counts per color by the total of foreground-pixels in the frame.
The result is an array with the frame's relative pixel-count per color, i.e., the share of that color in all foreground pixels.

\paragraph{Mapping of Color Counts to Classes}
To get from color count to classes, for each frame, we first assign the relative pixel-count of each color to a bin. However, a high number of bins might lead to both bad scalability and overfitting. Thus, we after the initial binning, we perform a bin refinement that finally assigns each color into a class.

Intuitively, the classes shall define whether a frame has more or less pixels of a certain color, though we are not limited to two classes, only. 

To assign classes, we first use an initial set of split-values that define the bin-ranges to have an initial set of bins.
Example: Assume two frames $f_1$,$f_2$ and a red color-count, only. The red-count of $f_1 = 20\%$, the red-count of $f_2 = 60\%.$ The split values $s$ are $0,10,50,100$, hence we find four possible bins per color. c($f_1$,$s$) returns $1$, c($f_2$,$s$) returns $2$. 
We then merge bins together according to their size and thereof define classes.

For an initial assignment of color-values to bins, we define the mapping $b:CxS \rightarrow B$ where $C$ is defined as above, the relative count per color, $S$ is a list of initial split values and $B = \mathbb{N}\in (0,|S|)^|C|$, which is one value \textit{s} for each color, where the relative color count is above the split value at position s but below the split value at position s+1. s is then the bin-number for this color.

For each frame in the test data-set and each color in the frame, we perform the color mapping into bins.
As a result, each frame is represented by a list of bin-numbers and a label. 
However, to compute a representative utility model that does not overfit, we next merge bins with too few samples into classes. 

\paragraph{Merging bins into classes using the minimum bin size}
\label{subsec:split_values}

\textit{Henriette: so maybe, it's actually supposed to be called minimum class size then??? if bins are the fine-grained version and merged into classes?? then all plots need to be re-named ... }

We introduce a minimum bin size (mbs). It is the minimum require share of all frames per bin. 
For example, a mbs of 5\% requires each bin to have at least 5\% of all samples from the training data-set. If this is not given, the bin is merged either with the next higher or next lower bin and the respective boundary removed. Once all merging is done, each color has an individual set of split-values (the bin boundaries) that match the respective color's distribution. 
The distributions of colors within the frames differ for each color. Hence, we further refine the class-assignment by adjusting the bin-sizes individually for each color.
Algorithm \ref{alg:bin_to_classes} shows how we merge bins that have too few samples into bigger bins.
The resulting merged, we call \textit{classes}. The smaller the mbs, the more classes per colors will be assigned. 

\begin{algorithm}
\caption{Merging bins to classes}
\label{alg:bin_to_classes}
\begin{algorithmic}[1]
\State split values $\leftarrow$ dict
\State minimumSamplesPerClass $\leftarrow$ numberOfSamples * mbs
\For{color in colors}:
    \State
    \State minBin = bin: min(|b(color,split-values) in bins|)
    \While {|minBin| < minimumSamplesPerClass}
    \State BinToMerge = bin with |bin| = min(upperBin, lowerBin)
    \State Merge bin and BinToMerge
    \State Remove split-value between merged bins
    \State minBin = bin: min(|b(color,split-values) in bins|)
    \EndWhile
    \State
    \State split values(colors) = new split values
\EndFor
\Return split values
\end{algorithmic}
\end{algorithm}

Thus, for each color we get a specific set of class-boundaries and thus an individual number of classes.

\subsubsection{Utility Computation}
After the class assignment and refinement, for each frame in the test data set, we have a mapping ${Class}^N \rightarrow L$ with ${Class} \in Classes_c$ for a color c, $N$ the total number of colors and $L \in {0,1}$ the frame's label.

To compute a frame's utility, the intuitive approach is to take the combination of each color as the frame's total class and compute this classes utility. 

However, we found out in preliminary evaluations that an approach that combines the classes of all colors to a joined class does not scale and requires a significantly large number of samples. Even after reducing the color-wise classes by applying Algorithm \ref{alg:bin_to_classes}, we still face about $2^{NxM}$ combinations (with N colors and M bins), thus classes in total.

Given the initial motivation that a developer should provide a set of labeled data for his query, an approach that generates such a large number of potential classes and thus requires even more samples to train an expressive classifier did not seem beneficial.

Hence, we propose a more approximate yet more scalable solution. The general idea is to compute a utility value for \textit{each color} individually and then assign the maximum value as the frame's overall utility. 

\subsubsection{Utility Computation and Assignment}
In detail, we  compute  the utility individually for each color and each class this color can have.  
As the  number of classes is defined dynamically  (see Subsection \ref{subsec:split_values}), the  number of utility values can be  different for each  color, too.

Each class of a color gets an individual utility value. We compute  them as shown in Equation \ref{eq:color_wise_utility}. For each color and each class in this color ($c_{color}$, we count the number of samples in this class with a positive label and divide it by the number of samples in this class in total.

\begin{equation}
\label{eq:color_wise_utility}
    u_(c, color) = \frac{\sum_{samples \in c_{color}: L(sample) = 1}}{ \sum_{samples \in c_{color}}} \forall colors
\end{equation}

A frame's utility is then  defined as in Equation \ref{eq:frame_utility}. We take the maximum utility value provided by a frame's colors. For example, in one frame the orange-class can have a high utility, while in another frame, red has the higher utility.

\begin{equation}
    \label{eq:frame_utility}
    u_f = max(u_{c_{color}}  | c(f,s_{color}))
\end{equation}

\subsection{Computing Threshold for Shedding Rates}
After these mapping steps, we have for each frame in the sample data-set a single utility value which is the maximum utility value of each frame's colors. 

To now compute a shedding rate, we sort the frames according to their utility and compute the cumulative distribution function (CDF).

Hence, our final model consists of three parts: The split values that define each color's classes, a utility model for each color, and the CDF that provides a distribution of utility values in the data stream.
Note that the CDF does not have a utility value for any possible x-value. Depending on the number of different utility values in the finally mapped list of frames, the CDF is a step-function with one step per utility value.

To shed a specific rate, the load shedder determines a utility threshold \textit{u} and sheds all input frames whose utility does not exceed this threshold. 

The shedder with a required shedding rate \textit{r} therefore first picks the respective threshold from the CDF: It iterates over the CDF until it finds the utility value \textit{u} for which holds: CDF(r') = u |r'>=r. I.e., it picks the utility value that maps to the smallest share of frames that equals or exceeds \textit{r}.


\subsection{Using the Utility Threshold at Runtime}
At runtime we determine a frame's utility and compare it against the load shedder's threshold: The algorithm thus performs the following tasks for each incoming frame:

\begin{enumerate}
    \item Apply f and b on the frame's H-histogram to get the respective class for each color. For b, use the split values provided by the model.
    \item Look up the utility for each color using the color's determined class.
    \item Take the maximum of all color's utilities.
    \item If the maximum is below \textit{u}, shed the frame, else forward it for processing.
\end{enumerate}

\subsection{Dynamic Adaptation of Utility Threshold}
\subsubsection{Monitoring current performance metrics}
\begin{itemize}
\item Per frame latency at every query operator
\item Actual selectivity of load shedder
\end{itemize}

\subsubsection{Determining the right threshold}
\begin{enumerate}
\item Use observed latency values at operators to estimate the maximum throughput that can be sustained by the query.
\item Use a history of observed load-shedding selectivity to estimate the relationship between the set drop ratio and the observed value.
\end{enumerate}

==> contents/overview.tex <==
\section{Template Overview}
As noted in the introduction, the ``\verb|acmart|'' document class can
be used to prepare many different kinds of documentation --- a
double-blind initial submission of a full-length technical paper, a
two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
journal article, a SIGCHI Extended Abstract, and more --- all by
selecting the appropriate {\itshape template style} and {\itshape
  template parameters}.

This document will explain the major features of the document
class. For further information, the {\itshape \LaTeX\ User's Guide} is
available from
\url{https://www.acm.org/publications/proceedings-template}.

\subsection{Template Styles}

The primary parameter given to the ``\verb|acmart|'' document class is
the {\itshape template style} which corresponds to the kind of publication
or SIG publishing the work. This parameter is enclosed in square
brackets and is a part of the {\verb|documentclass|} command:
\begin{verbatim}
  \documentclass[STYLE]{acmart}
\end{verbatim}

Journals use one of three template styles. All but three ACM journals
use the {\verb|acmsmall|} template style:
\begin{itemize}
\item {\verb|acmsmall|}: The default journal template style.
\item {\verb|acmlarge|}: Used by JOCCH and TAP.
\item {\verb|acmtog|}: Used by TOG.
\end{itemize}

The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
\begin{itemize}
\item {\verb|acmconf|}: The default proceedings template style.
\item{\verb|sigchi|}: Used for SIGCHI conference articles.
\item{\verb|sigchi-a|}: Used for SIGCHI ``Extended Abstract'' articles.
\item{\verb|sigplan|}: Used for SIGPLAN conference articles.
\end{itemize}

\subsection{Template Parameters}

In addition to specifying the {\itshape template style} to be used in
formatting your work, there are a number of {\itshape template parameters}
which modify some part of the applied template style. A complete list
of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

Frequently-used parameters, or combinations of parameters, include:
\begin{itemize}
\item {\verb|anonymous,review|}: Suitable for a ``double-blind''
  conference submission. Anonymizes the work and includes line
  numbers. Use with the \verb|\acmSubmissionID| command to print the
  submission's unique ID on each page of the work.
\item{\verb|authorversion|}: Produces a version of the work suitable
  for posting by the author.
\item{\verb|screen|}: Produces colored hyperlinks.
\end{itemize}

This document uses the following string as the first command in the
source file:
\begin{verbatim}
\documentclass[sigconf]{acmart}
\end{verbatim}

\section{Modifications}

Modifying the template --- including but not limited to: adjusting
margins, typeface sizes, line spacing, paragraph and list definitions,
and the use of the \verb|\vspace| command to manually adjust the
vertical spacing between elements of your work --- is not allowed.

{\bfseries Your document will be returned to you for revision if
  modifications are discovered.}

\section{Typefaces}

The ``\verb|acmart|'' document class requires the use of the
``Libertine'' typeface family. Your \TeX\ installation should include
this set of packages. Please do not substitute other typefaces. The
``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
as they will override the built-in typeface families.

\section{Title Information}

The title of your work should use capital letters appropriately -
\url{https://capitalizemytitle.com/} has useful rules for
capitalization. Use the {\verb|title|} command to define the title of
your work. If your work has a subtitle, define it with the
{\verb|subtitle|} command.  Do not insert line breaks in your title.

If your title is lengthy, you must define a short version to be used
in the page headers, to prevent overlapping text. The \verb|title|
command has a ``short title'' parameter:
\begin{verbatim}
  \title[short title]{full title}
\end{verbatim}

\section{Authors and Affiliations}

Each author must be defined separately for accurate metadata
identification. Multiple authors may share one affiliation. Authors'
names should not be abbreviated; use full first names wherever
possible. Include authors' e-mail addresses whenever possible.

Grouping authors' names or e-mail addresses, or providing an ``e-mail
alias,'' as shown below, is not acceptable:
\begin{verbatim}
  \author{Brooke Aster, David Mehldau}
  \email{dave,judy,steve@university.edu}
  \email{firstname.lastname@phillips.org}
\end{verbatim}

The \verb|authornote| and \verb|authornotemark| commands allow a note
to apply to multiple authors --- for example, if the first two authors
of an article contributed equally to the work.

If your author list is lengthy, you must define a shortened version of
the list of authors to be used in the page headers, to prevent
overlapping text. The following command should be placed just after
the last \verb|\author{}| definition:
\begin{verbatim}
  \renewcommand{\shortauthors}{McCartney, et al.}
\end{verbatim}
Omitting this command will force the use of a concatenated list of all
of the authors' names, which may result in overlapping text in the
page headers.

The article template's documentation, available at
\url{https://www.acm.org/publications/proceedings-template}, has a
complete explanation of these commands and tips for their effective
use.

Note that authors' addresses are mandatory for journal articles.

\section{Rights Information}

Authors of any work published by ACM will need to complete a rights
form. Depending on the kind of work, and the rights management choice
made by the author, this may be copyright transfer, permission,
license, or an OA (open access) agreement.

Regardless of the rights management choice, the author will receive a
copy of the completed rights form once it has been submitted. This
form contains \LaTeX\ commands that must be copied into the source
document. When the document source is compiled, these commands and
their parameters add formatted text to several areas of the final
document:
\begin{itemize}
\item the ``ACM Reference Format'' text on the first page.
\item the ``rights management'' text on the first page.
\item the conference information in the page header(s).
\end{itemize}

Rights information is unique to the work; if you are preparing several
works for an event, make sure to use the correct set of commands with
each of the works.

The ACM Reference Format text is required for all articles over one
page in length, and is optional for one-page articles (abstracts).

\section{CCS Concepts and User-Defined Keywords}

Two elements of the ``acmart'' document class provide powerful
taxonomic tools for you to help readers find your work in an online
search.

The ACM Computing Classification System ---
\url{https://www.acm.org/publications/class-2012} --- is a set of
classifiers and concepts that describe the computing
discipline. Authors can select entries from this classification
system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
commands to be included in the \LaTeX\ source.

User-defined keywords are a comma-separated list of words and phrases
of the authors' choosing, providing a more flexible way of describing
the research being presented.

CCS concepts and user-defined keywords are required for for all
articles over two pages in length, and are optional for one- and
two-page articles (or abstracts).

\section{Sectioning Commands}

Your work should use standard \LaTeX\ sectioning commands:
\verb|section|, \verb|subsection|, \verb|subsubsection|, and
\verb|paragraph|. They should be numbered; do not remove the numbering
from the commands.

Simulating a sectioning command by setting the first word or words of
a paragraph in boldface or italicized text is {\bfseries not allowed.}

\section{Tables}

The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
high-quality tables.

Table captions are placed {\itshape above} the table.

Because tables cannot be split across pages, the best placement for
them is typically the top of the page nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and the
table caption.  The contents of the table itself must go in the
\textbf{tabular} environment, to be aligned properly in rows and
columns, with the desired horizontal and vertical rules.  Again,
detailed instructions on \textbf{tabular} material are found in the
\textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed output of
this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more
desirable. Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.

\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}

Always use midrule to separate table header rows from data rows, and
use it only for this purpose. This enables assistive technologies to
recognise table headers and support their users in navigating tables
more easily.

\section{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of the three are
discussed in the next sections.

\subsection{Inline (In-text) Equations}
A formula that appears in the running text is called an inline or
in-text formula.  It is produced by the \textbf{math} environment,
which can be invoked with the usual
\texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
and structures, from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
examples of in-text equations in context. Notice how this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols and
structures available in \LaTeX\@; this section will just give a couple
of examples of display equations in context.  First, consider the
equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\section{Figures}

The ``\verb|figure|'' environment should be used for figures. One or
more images can be placed within a figure. If your figure contains
third-party material, you must clearly identify it as such, as shown
in the example below.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{resources/sample-franklin}
  \caption{1907 Franklin Model D roadster. Photograph by Harris \&
    Ewing, Inc. [Public domain], via Wikimedia
    Commons. (\url{https://goo.gl/VLCRBB}).}
  \Description{A woman and a girl in white dresses sit in an open car.}
\end{figure}

Your figures should contain a caption which describes the figure to
the reader.

Figure captions are placed {\itshape below} the figure.

Every figure should also have a figure description unless it is purely
decorative. These descriptions convey what’s in the image to someone
who cannot see it. They are also used by search engine crawlers for
indexing images, and when images cannot be loaded.

A figure description must be unformatted plain text less than 2000
characters long (including spaces).  {\bfseries Figure descriptions
  should not repeat the figure caption – their purpose is to capture
  important information that is not already provided in the caption or
  the main text of the paper.} For figures that convey important and
complex new information, a short text description may not be
adequate. More complex alternative descriptions can be placed in an
appendix and referenced in a short figure description. For example,
provide a data table capturing the information in a bar chart, or a
structured list representing a graph.  For additional information
regarding how best to write figure descriptions and why doing this is
so important, please see
\url{https://www.acm.org/publications/taps/describing-figures/}.

\subsection{The ``Teaser Figure''}

A ``teaser figure'' is an image, or set of images in one figure, that
are placed after all author and affiliation information, and before
the body of the article, spanning the page. If you wish to have such a
figure in your article, place the command immediately before the
\verb|\maketitle| command:
\begin{verbatim}
  \begin{teaserfigure}
    \includegraphics[width=\textwidth]{sampleteaser}
    \caption{figure caption}
    \Description{figure description}
  \end{teaserfigure}
\end{verbatim}

\section{Citations and Bibliographies}

The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

The bibliography is included in your source document with these two
commands, placed just before the \verb|\end{document}| command:
\begin{verbatim}
  \bibliographystyle{ACM-Reference-Format}
  \bibliography{bibfile}
\end{verbatim}
where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
suffix, of the \BibTeX\ file.

Citations and references are numbered by default. A small number of
ACM publications have citations and references formatted in the
``author year'' style; for these exceptions, please include this
command in the {\bfseries preamble} (before the command
``\verb|\begin{document}|'') of your \LaTeX\ source:
\begin{verbatim}
  \citestyle{acmauthoryear}
\end{verbatim}

  Some examples.  A paginated journal article \cite{Abril07}, an
  enumerated journal article \cite{Cohen07}, a reference to an entire
  issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
  monograph/whole book in a series (see 2a in spec. document)
  \cite{Harel79}, a divisible-book such as an anthology or compilation
  \cite{Editor00} followed by the same example, however we only output
  the series if the volume number is given \cite{Editor00a} (so
  Editor00a's series should NOT be present since it has no vol. no.),
  a chapter in a divisible book \cite{Spector90}, a chapter in a
  divisible book in a series \cite{Douglass98}, a multi-volume work as
  book \cite{Knuth97}, a couple of articles in a proceedings (of a
  conference, symposium, workshop for example) (paginated proceedings
  article) \cite{Andler79, Hagerup1993}, a proceedings article with
  all possible elements \cite{Smith10}, an example of an enumerated
  proceedings article \cite{VanGundy07}, an informally published work
  \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
    AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
  master's thesis: \cite{anisi03}, an online document / world wide web
  resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
  (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
  and (Case 3) a patent \cite{JoeScientist001}, work accepted for
  publication \cite{rous08}, 'YYYYb'-test for prolific author
  \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
  contain 'duplicate' DOI and URLs (some SIAM articles)
  \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
  multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
  couple of citations with DOIs:
  \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
  citations: \cite{TUGInstmem, Thornburg01, CTANacmart}. Artifacts:
  \cite{R} and \cite{UMassCitations}.

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
\begin{verbatim}
  \appendix
\end{verbatim}
and note that in the appendix, sections are lettered, not
numbered. This document has two appendices, demonstrating the section
and subsection identification method.

\section{SIGCHI Extended Abstracts}

The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
not in Word) produces a landscape-orientation formatted article, with
a wide left margin. Three environments are available for use with the
``\verb|sigchi-a|'' template style, and produce formatted output in
the margin:
\begin{itemize}
\item {\verb|sidebar|}:  Place formatted text in the margin.
\item {\verb|marginfigure|}: Place a figure in the margin.
\item {\verb|margintable|}: Place a table in the margin.
\end{itemize}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}

==> contents/problemstatement.tex <==
\section{Problem Statement}
\label{sec:problem_statement}

\todo{Do we really need this ?}

==> contents/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\subsection{Resource management in online video analytics}
Live video analytics is an extremely compute and network resource intensive application. Previous works have adopted two main approaches for managing the high resource requirements of this application - tuning the configuration of the input stream and video processing operators (e.g., frame rate, resolution, etc.) and early discard of uninteresting frames. Online adaptation of camera streams and video processing operators has been explored in \cite{videostorm,chameleon,soudain}. These works target scenarios where end-to-end latency of the order of sew seconds can be tolerated. Their primary objective is to optimize cost of resources needed for supporting all video streams while also maintaining high accuracy. Although these works differ from our proposed approach in terms of objectives, their technique can be adopted to work complementary to our proposed approach.
\par Multiple approaches have been taken for performing early discard of unnecessary video frames so that compute and network costs of streaming and processing them can be avoided. Glimpse \cite{glimpse} proposed a hardware-software addon that could use low-powered coarse-grained vision modalities to filter out frames irrelevant to the query at hand. FilterForward \cite{filterforward} consists of a base DNN whose intermediate layers' outputs are used by a per-application binary classifier that decided whether to filter out a frame or not. The EarlyDiscard strategy proposed in \cite{drones} uses an inexpensive DNN to perform filtering of frames. \cite{fastfiltering} uses a multi-stage pipeline of operators to detemine whether a frame is relevant to a query. Reducto \cite{reducto} makes use of difference in low-level visual features (such as pixels, edges, etc.) across consecutive frames to determine if processing the new frame would result in a difference in the query's result. 

==> contents/results.tex <==
\section{Evaluation Results}
\label{sec:evals}

\par Evaluation hypotheses
\begin{enumerate}
\item Utility function is able to compute utility value for frames from an unseen video (not in training set).
\item The utility value calculation is light-weight and imposes low overhead on edge devices.
\item The proposed control loop adapts to changing workload pattern and is able to meet application performance requirements without sacrificing accuracy.

\end{enumerate}


\textit{Henriette:  Update this text if evaluations change  accordingly. I wrote it with those experiments in mind we had discussed till sep 9th.}
In this section, we present the results of our evaluations. We conducted multiple experiements to show how we selected parameters, how the load shedder behaves in terms of quality, to what extend it hits the required shedding rate, and how ultimately shedding influences the queuing latency of the video streams.

\subsection{Data Set}
For the presented  evaluations, we trained the model with different parameters (discussed below) and with a training data-set of video streams from multiple cameras. We then conducted all experiments using the trained models and and a test data-set with new streams but from the same cameras. 

\textit{refine accordingly.}

\subsection{Queries}

\textit{describe red, or, and query.}

In the test data-set used, the data for the "RED" query had about 25\% matches, the data for the "OR" query 20\%, and the data for the "AND" query only 1\%. 

\subsection{Metrics used}
We discuss our solution based on two major metrics: The false-negatives rate and the deviation of the actual to the required ratio.

\paragraph{False-negatives rate}
Assume the set of all frames that match the query is denoted as ${F^+}$. 
Then those frames that match but are falsely dropped by the shedder are denoted as ${F^+_d}$.

The false-negatives rate is thus $\frac{F^+_d}{F^+}$, telling the share of all matches that have been falsely dropped by the shedder.

We discuss our solution with regards to quality using this metric.


\paragraph{Deviation of achieved to required rate}
The achieved shedding rate can deviate from the required rate for two reasons: First, the distribution of $F^+$ in the training data-set can differ from the distribution in the test data-set. Thus, the CDF returns a utility value \textit{u} for a given rate \textit{r}, because this is the threshold where r\% of the training frames had a utility of u or less. However, if in the test data-set, e.g. $F^+$ is smaller, hence fewer frames have a high utility, more frames than expected would be shed, leading to a higher actual shedding rate.

Second, the CDF does not provide a utility value for every possible rate. It rather picks the value as threshold that is next higher to the required rate $r$. So even if the distributions were the same in test and training data, it is possible to shed slightly more than $r$. 

To this end, we measured the actual shedding rate $r_a$ for each experiment and compute how much it deviates from the required shedding rate $r$ that we specified for the experiment. The smaller this deviation the better, as $r$ will be determined with a latency bound in mind, hence the if $d_r = r_a$ - $r$ is negative, i.e., the shedder sheds too little, the bound might be violated. If $r_a$ -$r$ is positive, the shedder might shed unnecessarily much which decreases quality more than necessary. 

We will therefore discuss the experiments also with regards to this deviation, where it holds that the smaller the better. 

\textit{Somewhere add the control-loop idea. if the $abs(d_r)$ is too high, update ratio.}

\begin{figure*}%[!htb]
% all plots in "compute_false_positives_and_negatives.py"
% for function see respective comment in mini-page
    \centering
    \begin{minipage}{.3\textwidth}
        %plot_fn
        \centering
        \includegraphics[width=\linewidth]{resources/red/false-negatives_over_mbs.png}
        \caption{False Negatives "RED" for  different MBS}
        \label{fig:fn_red_mbs}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    %plot_fn
        \centering
        \includegraphics[width=\linewidth] {resources/or/false-negatives_over_mbs.png}
        \caption{False negatives "OR" for different MBS}
        \label{fig:fn_or_mbs}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    %plot_fn
        \centering
        \includegraphics[width=\linewidth]{resources/and/false-negatives_over_mbs.png}
        \caption{False negatives "AND" for different MBS}
        \label{fig:fn_and_mbs}
    \end{minipage}%
    \\
    \begin{minipage}{.3\textwidth}
    %plot_ratios_by_mbs
        \centering
        \includegraphics[width=\linewidth]{resources/red/ratios_by_mbs.png}
        \caption{Ratio deviation "RED"}
        \label{fig:ratio_red_mbs}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    %plot_ratios_by_mbs
        \centering
        \includegraphics[width=\linewidth] {resources/or/ratios_by_mbs.png}
        \caption{Ratio deviation "OR"}
        \label{fig:ratio_or_mbs}
    \end{minipage}%
    %plot_ratios_by_mbs
        \begin{minipage}{.3\textwidth}
        \centering
        \includegraphics[width=\linewidth]{resources/and/ratios_by_mbs.png}
        \caption{Ratio deviation"AND"}
        \label{fig:ratio_and_mbs}
    \end{minipage}%
\end{figure*}

\subsection{Selection of the optimal minimum bin size}
The miminum bin size (mbs) controls how many classes per color our algorithm generates. The smaller the mbs, the more classes there are. A well-chosen mbs thus balances scalability, precision of the model, and overfitting.

Recall that mbs is relative value, i.e., an mbs of 0.1 requires  for each  class to have at least  10\% of  the total number of samples (or 0.1*total).

Before we present our quality-evaluations for fine-grained shedding rates, we first show evaluations over three shedding rates but  for different mbs. 
The goal is to gain an understanding what a benefitial mbs-value is for the upcoming evaluations. 

Figures \ref{fig:fn_red_mbs} to \ref{fig:ratio_and_mbs} show how the load shedder performs for our test data-set.

\paragraph{Choosing mbs with regards to optimal quality}
Figures \ref{fig:fn_red_mbs} to \ref{fig:fn_and_mbs} show the quality achieved for different mbs (x-axis) and the shedding rates 0.3, 0.5, and 0.7 for all three queries. 

For the "RED"-query, we see that quality decreases (false negatives raise) for a mbs above 0.2 The same holds for the "OR" query. For the "AND" query we see that only for high shedding ratios the bigger mbs have a negative effect. This is explained by the very few matches in the system that permit the shedder to shed much without producing any false positives. 

We also see only small differences in the quality for values lower than 0.2. As a bigger mbs leads to fewer classes and is thus less prone to overfitting or poor scalability, we choose 0.2 as the mbs for the following experiments and compare it's results to mbs 0.3.

Finally, especially for the "OR" query we see that a careful choice of mbs is important as there cannot always be shown a clear trend, such as bigger bin size leads to worse quality. 

\paragraph{Choosing mbs with regards to rate deviation} 
Figures \ref{fig:ratio_red_mbs} to \ref{fig:ratio_and_mbs} show how well the load shedder matched the required ratio. We see for smaller mbs in all three queries that the shedder does not always shed enough (negative deviation). This makes the system prone to latency violations and thus strengthens our choice of 0.2 for mbs. 

\subsection{Evaluation for different shedding rates}

\begin{figure*}%[!htb]
% all plots in "compute_false_positives_and_negatives.py"
% for function see respective comment in mini-page
    \centering
    \begin{minipage}{.3\textwidth}
    % plot_mbs_lines with y-axis parameter "false_negatives
        \centering
        \includegraphics[width=\linewidth]{resources/red/fn.png}
        \caption{False Negatives "RED"}
        \label{fig:fn_red}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    % plot_mbs_lines with y-axis parameter "false_negatives
        \centering
        \includegraphics[width=\linewidth] {resources/or/fn.png}
        \caption{False Negatives "OR"}
        \label{fig:fn_or}
    \end{minipage}%
        \begin{minipage}{.3\textwidth}
    % plot_mbs_lines with y-axis parameter "false_negatives
        \centering
        \includegraphics[width=\linewidth]{resources/and/fn.png}
        \caption{False Negatives "AND"}
        \label{fig:fn_and}
    \end{minipage}%
    \\
    \begin{minipage}{.3\textwidth}
    % plot_mbs_lines with y-axis parameter "better_than_random"
        \centering
        \includegraphics[width=\linewidth]{resources/red/performance.png}
        \caption{Performance "RED"}
        \label{fig:performance_red}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    % plot_mbs_lines with y-axis parameter "better_than_random"
        \centering
        \includegraphics[width=\linewidth] {resources/or/performance.png}
        \caption{Performance "OR"}
        \label{fig:performance_or}
    \end{minipage}%
        \begin{minipage}{.3\textwidth}
        % plot_mbs_lines with y-axis parameter "better_than_random"
        \centering
        \includegraphics[width=\linewidth]{resources/and/performance.png}
        \caption{Performance "AND"}
        \label{fig:performance_and}
    \end{minipage}%
    \\
    \begin{minipage}{.3\textwidth}
    % plot_ratios
        \centering
        \includegraphics[width=\linewidth]{resources/red/ratios.png}
        \caption{Ratio Deviation "RED"}
        \label{fig:ratios_red}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    % plot_ratios
        \centering
        \includegraphics[width=\linewidth] {resources/or/ratios.png}
        \caption{Ratio Deviation "OR"}
        \label{fig:ratios_or}
    \end{minipage}%
    \begin{minipage}{.3\textwidth}
    % plot_ratios
        \centering
        \includegraphics[width=\linewidth]{resources/and/ratios.png}
        \caption{Ratio Deviation "AND"}
        \label{fig:ratios_and}
    \end{minipage}%
\end{figure*}

In Figures \ref{fig:fn_red} to \ref{fig:ratios_and}, we show the behavior of our load shedder for the given experiment set up over a wide range of shedding rates.
In particular, we show three different properties: \enquote{How does the quality change for different rates and queries (Figures \ref{fig:fn_red} to \ref{fig:fn_and})?}, \enquote{How much better than a random, i.e., uninformed shedder, does our load shedder behave with regards to quality (Figures \ref{fig:performance_red} to \ref{fig:performance_and})?}, and \enquote{How well does the shedder meet the required rate, hence sheds enough to avoid SLA-violations yet not shed too much to avoid unnecessary quality decreases (Figures \ref{fig:ratios_red} to \ref{fig:ratios_and})?}. 

The required ratios for all experiments in this section were 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9.

\subsubsection{Quality}
First, we discuss the false-negative rates for all three queries (Figures \ref{fig:fn_red} to \ref{fig:fn_and}). 
On the x-axis we show the actual shedding rate, on the y-axis the false-negative rate, i.e., the share of all matches that has falsely been dropped.
As a benchmark for the quality discussion, we executed the experiments with a random shedder, too. So in each of the three figures  we provide the false negative rate for the selected mbs 0.2, the worse mbs 0.3 to compare, and the random runs. As expected, the random shedder sheds proportionally as many matches as it sheds frames in total.

For the "RED" query, we observe that the difference between mbs 0.2 and 0.3 is small. We further observe for all three queries that for a high shedding rate (0.9) our load shedder has an actual rate of 1, hence sheds all events and thus also all matches.

For the "OR" and the "AND" query, we see for shedding rates greater than 0.5 a significant quality improvement of the selected mbs compared to the worse 0.3, as the blue curve is below the orange - and of course below the green - one. 

Hence, we can summarize that our approach is able to, first, perform with good quality if the mbs is chosen carefully, and second, outperforms in both cases (0.2 and 0.3 mbs) the random shedder.

To better understand the latter point, we further show the quality improvement over random in the following three figures  (Figures \ref{fig:performance_red} to \ref{fig:performance_and}).

\subsubsection{Improvement over random}
The figures show on the x-axis again the actual shedding rate. On the y-axis, they show the relative quality improvement over a random, i.e., uninformed shedder. The goal is to show to how much "better than random" our shedder is. 
We compute the y-axis $q$ therefore as given in Equation \ref{eq:quality_improvement}.$r_a$ is the actual shedding ratio, $fn$ is the false negative rate, i.e., the share of matches of all matches that has falsely been shed.

If $q$ is 0, the shedder sheds the same share of matches in all matches than the share of shed events in all events. Hence, we aim for q > 0 which tells that the shedder is able to shed proportionally more "useless" frames first and keeps the matches.  

\begin{equation}
    \label{eq:quality_improvement}
    q = r_a - fn / r_a 
\end{equation}

It becomes visible that for all three queries, our load shedder performs better than random for all shedding ratios except for 0.9. It becomes further visible that again, mbs 0.2 outperforms mbs 0.3 as expected. 

\subsubsection{Deviation of required ratio}
As introduced, we thrive towards a solution that matches the required ratio as good as possible. Figures \ref{fig:ratios_red} to \ref{fig:ratios_and} show how well the shedder achieves this goal. On the x-axis, we show the required rate, on the y-axis, we show the deviation of the achieved rate from the required one. The top row shows the deviations for mbs 0.2, the lower row the deviations for mbs 0.3.

It becomes visible that in almost all cases, the shedder tends to either hit the ratio or sheds too much. Thus, to keep a latency goal, both configurations (mbs 0.2 and mbs 0.3) are legible. We, however, further see that mbs 0.2 has in most cases a lower deviation except for a shedding rate of 0.6, where mbs 0.3 matches the rate for any given query as opposed to mbs 0.2 which has a small deviation.

\subsection{Notes for conclusion}
\textit{Henriette: Here just a few bullets what could come into a conclusion of the evaluation}

\begin{itemize}
    \item Shedder performs also well for query with small set of matches - is able to keep those until it really has to shed everything.
    \item Shedder outperforms random - even for poorly set parameters (mbs 0.3)
    \item picking the right mbs is still important for good quality.
    \item short summary of the discussion what happens if the deviation is too high / low
    \item ... 
\end{itemize}
